Structural Abstraction as an Inductive Bias for Non-Stationary Language Model Training

A foundational principle in cognitive science holds that intelligent agents do not learn by storing experiences as isolated instances, but by forming abstract schemas that capture relational structure shared across situations. Even though this claim is well supported by behavioral and neuroimaging studies, its role as a computational training signal in language models remains underexplored. We target this gap in the setting of non-stationary language model training, asking does biasing learning toward structural abstraction reduce catastrophic interference and improve relational generalization as predicted by human results? To study this question, we introduce Abstraction-Augmented Training (AAT), a lightweight loss-level modification that jointly optimizes over concrete instances and their structural abstractions, and two benchmarks, the Relational Cycle Benchmark (RCB) and the Narrative Abstraction Benchmark (NAB). These resources operationalize core cognitive constructs: entity masking as a computational analog of relational alignment, and proverbs as vehicles for implicit abstract meaning that must be inferred across surface-dissimilar situations. Our empirical results demonstrate that AAT consistently reduces forgetting and improves generalization in a pattern that aligns with cognitive predictions for schema-based learning. Beyond the practical implications for continual learning, these results offer preliminary computational evidence that structural abstraction is a signal for stable learning in non-stationary environments.

==> plots_and_tables/random_seeds_table.tex <==
\begin{table}[t]
\centering
\caption{effect of data order}
\label{tab:order-effect}
\resizebox{0.9\columnwidth}{!}{ 


\begin{tabular}{lccc}

Method & $Acc_{cumul}^{unknown}$ & $Acc_{cumul}^{known}$ & $Acc_{cumul}^{all}$ \\
\hline
no\_abstract & 0.3651 ± 0.0382 & 0.5312 ± 0.0018 & 0.4791 ± 0.0134 \\
buffer & 0.3775 ± 0.0061 & 0.5483 ± 0.0032 & 0.4949 ± 0.0041 \\
abstract & 0.3763 ± 0.0323 & 0.5510 ± 0.0058 & 0.4962 ± 0.0063 \\
\end{tabular}

}


\end{table}
